"When He Feels Cold, He Goes to the Seahorse"-Blending Generative AI into Multimaterial Storymaking for Family Expressive Arts Therapy

Storymaking, as an integrative form of expressive arts therapy, is an effective means to foster family communication. Yet, the integration of generative AI as expressive materials in therapeutic storymaking remains underexplored. And there is a lack of HCI implications on how to support families and therapists in this context. Addressing this, our study involved five weeks of storymaking sessions with seven families guided by a professional therapist. In these sessions, the families used both traditional art-making materials and image-based generative AI to create and evolve their family stories. Via the rich empirical data and commentaries from four expert therapists, we contextualize how families creatively melded AI and traditional expressive materials to externalize their ideas and feelings. Through the lens of Expressive Therapies Continuum (ETC), we characterize the therapeutic implications of AI as expressive materials. Desirable interaction qualities to support children, parents, and therapists are distilled for future HCI research.

==> texfiles/5-Findings1.tex <==
\section{Findings 1}

\subsection{Understanding AI-infused Storymaking Expressive Art Therapy}
In this section, we examined how family members engaged in storymaking-based expressive art therapy using AI and diverse physical materials. We employ the four activities as a lens to analyse the involvement of parents and children in the therapeutic settings, as well as the potential therapeutic functions. A summary of our results is shown in (see \autoref{fig:finding1}).

In terms of character making, most children and parents chose to use drawing or knead clay to create their own characters. Additionally, some children incorporated their personal toys into the stories, utilizing them as characters through externalized metaphors~\cite{perrow2008healing}. For example, P8 used a dinosaur toy as an obstacle metaphor(see \autoref{fig:finding1}~\circled{6}). At the same time, certain story characters could project children's emotional and inner thoughts:\qt{children have a consistent character, which could be regarded as a projection of the child's own self.[…]For the child, the primary focus is on how they project these characters into their own stories~(T3)}. 

Regarding to scene and object making, in addition to drawing, building with LEGO® and making with colored clay, children used AI-printed materials and non-woven fabric to make collages, which were also one of main ways to build scenes(see \autoref{fig:finding1}~\circled{7} and \circled{8}). Further, some children made their own scenes by mixing AI-printed materials with physical materials~(wool, colored clay). In the process of constructing scenes/objects, most children mapped their own life experience scenes by constructing metaphoric representation. Also, according to expressive art therapy theory, the process of ordering and structuring scenes might be associated with emotional content~\cite{hinz2019expressive}.

Concerning storymaking and storytelling, P13 tended to employ AI-printed materials as story characters and blue cardboard as a scene to tell stories through moving the AI-printed materials back and forth(see \autoref{fig:finding1}~\circled{13}). Also, role-playing(see \autoref{fig:finding1}~\circled{15} and \circled{16}) was used by our family members through AI-printed materials, character tokens or their personal toys, which might provide opportunities to project qualities of themselves and practice perspective taking~\cite{jennings2005embodiment}. Finally, body movement performance was founded in our study(see \autoref{fig:finding1}~\circled{17}) through idea forming, rehearsal and showing, which served as an efficient means for initial exploration and re-exploration of a challenge~\cite{jones1991dramatherapy}.

With regard to sharing and reflection, in addition to sharing the storybooks created by AI during the activities, they also shared and developed their stories beyond the activities. For example, some children share their storybooks with family members(see \autoref{fig:finding1}~\circled{18} and \circled{19}); Children played with character tokens at home and made crafts based on character tokens(see \autoref{fig:finding1}~\circled{20}, \circled{21} and \circled{22}); Children used AI-printed materials to make new storybooks at home(see \autoref{fig:finding1}~\circled{23} and \circled{24}).

\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{images/finding1.jpeg}
  \vspace{-4mm}
  \caption{Parents and Children Participated in the Storymaking Process in Four Activities.}
  \Description{Figure 1 portrays a family employing a palette of vibrant colors, specifically blue and green, to craft an eight-legged blue-ringed octopus on paper. Simultaneously, an AI-generated cartoon image emerges, featuring a one-eyed rendition of the captivating creature. In Figure 2, a child's artistic expression unfolds as spontaneous brushstrokes and formalized lines converge to give life to a regal purple Transformers. AI generated a cartoon purple Transformers, harmonizing with the child's imaginative strokes. In Figure 3, a child explores the realm of colorful structures, utilizing playful hues such as red, blue, yellow, and black. The juxtaposition of a snail adorned with blue headphones, alongside its AI-generated counterpart with oversized eyes and matching headphones, showcases the embodiment of a childlike aesthetic. Figure 4 captures the child's uninhibited use of differently colored clay(a hedgehog bedecked with a yellow rope knot.). Figure 5 features a green watermelon-shaped toy car, mirrored by an AI-generated image that seamlessly complements the child's creation. Figure 6 presents a menacing green dinosaur, mouth agape, brought to life through AI wizardry. Figure 7 unfolds a delightful scene where children, through collage, express the joyous tapestry of their kindergarten life. The children used soft pastel-colored non-woven fabric to make the scene of the kindergarten which placed two symmetrical trees at the entrance of the kindergarten. Different AI-generated characters of paper cutout are neatly arranged together. In Figure 8, a child utilized collage to depict a blue-ringed octopus dwelling in the profound, shadowy depths of an oceanic cave surrounded by vibrant seaweed. Figure 9 employs dark tones and scenes to evoke a profound emotional resonance, depicting blue clouds, pouring rain, yellow trucks, and black roads—a visual testament to heavy, depressing, or gloomy feelings. Figure 10 showcases a child's artistry with an eclectic blend of colors, fashioning a symmetrical and balanced Lego castle and clay park. Figure 13 shows a child telling a story to his parents. He uses artificial intelligence paper cutouts and blue cardboard to immersively tell stories that happen under the sea. Figure 14 shows two siblings sharing their own stories with each other. Figure 15 shows the child happily playing with the Transformers he brought from home and the character tokens generated by AI and improvising the story. Figure 16 presents a role-playing activity which a child, aided by AI-generated character cutouts, engages in role-playing with their mother, placing the character cutout on their forehead. Figure 16 shows that the daughter and mother were playing roles. The daughter was immersed in telling what happened in the story by placing the AI-generated paper cutout on her forehead. Figure 17 shows children using body performance to tell stories about Godzilla and Transformers with their parents. Figures 18 and 19 depict heartwarming moments through sharing physical storybooks with their father in their home. In Figure 20, a child is depicted integrating AI-generated character tokens with personal toys at home, facilitating interactions between the AI-generated characters and their toys. Figures 21 and 22 illustrate the imaginative prowess of children as they craft analogous characters from colored clay inspired by AI-generated character tokens. Moving forward to Figures 23 and 24, these snapshots capture the creative journey of children meticulously crafting their own storybooks using a blend of artificial intelligence materials and traditional art supplies. This process serves as a meaningful connection between their past and future energies through the medium of artistic creation.}
  \label{fig:finding1}
\end{figure*}

\subsection{Understanding Children's, Parents' and Therapists' Needs}
In this section, we focus on understand and support  the needs of children, parents, and therapists in the context of storymaking-based expressive art therapy, examined through the lens of HCI. We reported our findings clustered under the three themes~(see Table~\ref{tab:finding1need}):(1) Children's needs; (2) Parents' needs; and (3) Therapists' needs. 

\subsubsection{Children's Needs}
In our findings, we first reported how to support children's needs in storymaking-based expressive art therapy. We finally identified five themes: (1) Diverse Material for Creative Exploration and Expression; (2) Authentic Encounter with Reality; (3) Parental Involvement; (4) Sense of Accomplishment; (5) Renarration Beyond Activities.

\textbf{Diverse Material for Creative Exploration and Expression.} 
In our research, we found that one of the desired qualities for children who would like to be supported is diverse materials. Diverse materials can support in the following three aspects: (1) self-regulation and motor skills; (2) non-verbal expression; (3) creative empowerment.

First, it might empower children to enhance their self-regulation and motor skills. P5, for instance, demonstrated that clay can promote P8 to focus more on making his own things: \qt{while kneading clay, my son was really focused, seemingly unaffected by external happenings}. Further, P9 was extremely \qt{surprised} that P10 \qt{could make so many different kinds of small animals in a short time}. Homer et al. examined that fabric collages have the similar significant therapeutic benefit for clients\cite{homer2015piece}.

Second, it might empower children's non-verbal expression. Our findings indicated that certain parents were concerned that their children might not express their feelings through verbal communication:\qt{when I directly asked him how he felt, he didn't say it. He didn't like to express his feelings very much~(P3)}. Materials are a medium for emotional expression for children. As noted by P3, \qt{we engaged in joint painting using a marker pen. Initially, he created dotted lines regularly; after a while,  he scribbled circles wantonly. I think it is actually a kind of emotional release}. T4 explained that:"\qt{half of the children could tell stories in their drawings}.

Finally, it fosters creative empowerment in children. Children showed greater interest in creating new objects using physical materials:\qt{he used LEGO® to build a prison that time. He basically built it according to a blueprint. So, he rarely built such a thing creatively by himself~(P17)}. Creativity is an integral part of therapy which could allow individuals to express their feelings and experiences in non-verbal ways\cite{manheim1998relationship}, and promote self-actualization:\qt{the dynamics of the social world are in flux, and there are instances where our acquired knowledge and skills might not suffice to navigate these shifts. Nonetheless, our creativity equips us with the prowess to confront the unfamiliar~(T1)}.

\textbf{Authentic Encounter with Reality.} It is evident that authentic encounter with reality is an essential needs for our children participants. Authentic encounter with reality can facilitate two aspects: (1) the incorporation of real characters into stories; (2) the incorporation of personal objects into stories.

First, many parents talked about their children identifying themselves or their family members as story characters in their own stories. P11 mentioned that the most impressive experience was that the child made a\qt{purple fish} out of colored clay: \qt{P13 said at the time that he turned into a fish}. P11 added that:\qt{he said that the seahorse is the mother and the jellyfish is the father}. Children could project inner emotional state and externalize inner conflicts through story characters\cite{jennings2005embodiment}. Further, T1 highlighted that it could help children discover and understand unknown quality:\qt{some children might recognize their kindness and peaceful quality in the stories because they project themselves onto the characters}.

Second, we found that personal favorite toys for children were also integrated into their own stories. P11 reflected that:\qt{I have always been surprised by the turtle toy, I don't know what it means to him. He always carries this toy with him wherever he goes and holds it in his hand when he sleeps. So, the turtle character frequently appears in various his story scenes. This tortoise seems to offer him continuous companionship}. P17 believed that the toys create a connection with children:\qt{he loves toys very much. When these toys were integrated into his stories, he might perceive them as more than mere playthings, and thus the toy might connect with the child}. Children might use toys to represent their inner world and external experiences symbolically\cite{harvey1990dynamic}.

\textbf{Parental Involvement.} Our research reveals that parental involvement is also a desired quality for children. First, many parents noted that parents serve as a role model for positively influencing children's participation, e.g,\qt{when he observed me engaging in making, it could affect P4. I guess he felt mommy focused on making her own thing, and thus I should focus on making my own thing too~(P3)}. Children often learn by observing and imitating the behaviors of their parents\cite{minuchin2018families}. Parents' engagement could thus motivate children to embrace creative and expressive activities in therapeutic settings. 
In addition, we found that parents and children co-constructed common topics and integrated these topics into their stories. For instance, P11 described that: \qt{ocean themes are also of interest to his dad, including fried egg jellyfish, blue-ringed octopus, and more}. Forging topics of common interest can enhance communication between parents and children:\qt{in this common topic area, they can communicate and are really professional~(P11)}. 

\textbf{Sense of Accomplishment.} 
How to support children's sense of accomplishment in family expressive art therapy is also a desired quality for children. First, many parents reflected on children's joy at creating results that exceeded expectations. P1 stated that the sense of achievement came from the art works created by AI that exceed expectations:\qt{last time I asked her if she remembered the characters using clay. She said that the computer helped her make such a beautiful character. I asked her if she liked it, and she said she loved this character. She felt that she actually couldn't draw such a good-looking character}. T4 believed that:\qt{the relationship between the creator and his creation is also important in expressive art therapy. Thus, it is crucial to establish ownership over the outcomes generated by AI and the creators}. T1 added that \qt{many children would say that they made the storybooks, and they also came up with these characters}. Moreover, children were willing to share their own physical storybooks created by AI with family members or their own friends. For example, P11 shared that:\qt{He gets frustrated if he doesn't have anything to share every week. He will take his storybook to kindergarten to share it with others. Whenever he brought up the topic of AI storybooks with fellow children, they didn't know what he's talking about. He didn't know what AI was either, but he told his friends I was going to AI today}. Sharing might create a sense of togetherness and unity in supporting the child's growth and learning\cite{malti2012early}.

\textbf{Renarration Beyond Activities.} 
In our findings, one of interesting themes for children is renarration beyond activities. That means that many children employed the characters created by themselves to continue making new stories in home. P1 examined that P2 used the materials printed by AI to continue creating stories:\qt{she used those AI pictures to make this storybook again, and she will definitely add story plots after a while}. P10 not only used materials generated by AI, but also utilized physical materials from life:\qt{it happened to be the day after the Dragon Boat Festival. When I was cleaning her desk, I took out the AI-printed materials from the drawer and encouraged her to make a storybook together. When she first started cutting, I saw her cutting these AI-printed materials. Then, I told her that there was foam in the express package, and she said that this foam could be used to make three-dimensional glue~(P9)}. In the broader context, it can facilitate creative explorations and express their experience for children\cite{panjwani2017constructing}.

\subsubsection{Parent's Needs}
 In our study, we proposed four theme for parents: (1) Discovering New Aspects of Children; (2) Learn from the Therapist; (3) Reflection in Therapeutic Storymaking; (4 )Family Meaning Co-constructing.
 
\textbf{Discovering New Aspects of Children.}
An interesting theme emerged from the parents' perspective to support is that parents need to discover new aspects of children through family storymaking. Specifically, parents can uncover the following three novel facets of their children through stories: (1) discovering children's demands for parents; (2) discovering children's less noticeable life experiences; (3) discovering children's strengths.

First, many parents could uncover children's demands for parents within the family unit through their stories. For example, P11 talked about her child's demands for father and mother through story characters as a metaphorical symbol: \qt{To the seahorse~(created by the child), a seahorse might be the mother. So when the purple fish~(created by the child) felt cold, he went to the seahorse because the seahorse gave him a sense of security}. On the contrary, for P12's dad, \qt{the fried egg jellyfish~(created by the father) was not mentioned at all. The fried egg jellyfish exists in a floating state, devoid of a fixed abode and without the need for sleep. It simply drifts along~(P11)}. It might support parents in uncovering children's demands within their family structure, leading to enhanced insight into how family members identify their roles~\cite{kwiatkowska1967family}.

Second, we found that parents can discover children's less noticeable life experiences through stories. Children incorporated their own real life experiences into their own stories. P9 demonstrated that she could understand P10's experience and feelings in kindergarten from P10's story:\qt{through the activities, she first thought of the theme of kindergarten, because she may feel that she spends most of her time in kindergarten. Then, I realized that she might feel that kindergarten life for her is happy and enjoyable}. Storytelling might be a powerful way to help parents make sense of children's experiences and their identities\cite{langellier2004storytelling}. 

Finally, parents in our study talked about their experiences of uncovering their children's strengths through stories. P3 reflected that she might be unaware of the heroic qualities that reside within P4:\qt{I didn't expect that he would want to help me find the gem because it was lost. From my point of view, he might lose his temper, but the character he created was a heroic character. Internally, he nurtures the conviction that he possesses a heroic disposition. Unfortunately, I may not have provided opportunities to showcase this aspect, causing me to never realize the existence of his inner hero}. Parents can learn to use these strengths of their children to help them solve future difficulties though storytelling:\qt{you(P1) can incorporate actual experiences into Xixi's stories. These stories integrated numerous strengths of Xixi. she will come to appreciate the abundance of strengths she holds, eventually internalizing them as a core aspect of her being.This, in turn, may empower her to leverage strengths to face these difficulties~(T1)}. Also, T1 explained the therapeutic meaning about observing their children's new characteristics:\qt{parents need to amplify their children's strengths consistently, transforming them into shining points}. 

\textbf{Learn from the Therapist.} 
Another interesting theme that emerged from several parents was that they could learn how the therapist interacted with their children. Parents first learn how to accept and minimize judgment towards their children. For instance, P3 expressed being deeply moved by T1's mode of communication with the child:\qt{he often used some offensive languages, such as saying that you are so stupid. I remember one time I saw T1 asking him, to whom do you think you would say such things? The child said that he said this to his good friends or close people}. The non-judgmental approach for parents can help children foster self-expression and emotional exploration\cite{isis2015positive}. Further, we found that parents can learn how to nurture children's imagination, e.g, \qt{sometimes we deny our children's wild imagination. I would question how it is possible to stay on the clouds for 40 minutes. I think it was great when the therapist guided her to imagine~(P9)}. Following children's natural imagination might foster family connection~\cite{soule2008creative}.

\textbf{Reflection in Therapeutic Storymaking.} In our study, many parents expressed that they tended to reflect their family dynamics through the activities. There are three aspects: (1) reflect on their roles; (2) reflect their family interactions; (3) reflect on their own results-oriented expectations.

First, through this activity, some parents can reflect on their roles at home in the past. For example, P1 examined that parents plays a supervising roles at home:\qt{within the domestic context, I often find myself urging her to expedite tasks. In truth, the predominant role I fulfill within our home is that of her supervisor}. Further, P3 reflected on her current role and prepared to make changes:\qt{at home, I paid more attention to my children's affairs, often taking on a controlling or guiding role. I will have more time to do my own things in the future}. Parents’ reflection on roles can fluidly change their family roles and increase family flexibility~\cite{olson2000circumplex}. 

Further, many parents expressed that they can reflect their family interactions in the past through the activity:\qt{ in fact, we seldom engage in playtime with our two children. They tend to amuse themselves individually or seek playmates. It seems that families engage in few collaborative play activities together~(P5)}. Further, P9 realized that she needed to \qt{spend more time with P10 in the future}. Parents’ reflection on family interactions might promote more time together~\cite{olson2000circumplex}.

Finally, many parents in our research reflected on their own results-oriented expectations. Many parents reflected that their excessive pursuit of intricate story plots during storymaking, e.g,\qt{in the process of co-creation together, I always felt that P2's story plot was too simple. That means that her story plots had no twists and turns. Yet, I immediately realized that this could also be an authentic reflection of her inner world~(P1)}. Further, P3 reflected on the process from not accepting to accepting children's stories:\qt{In the initial stages, I was resistant to accepting his outcomes. It seemed that if we were going to make a story, it must be a perfect story. Yet, I gradually embraced the outcome. Given his age, it's entirely reasonable for him to create stories in this manner}. T1 explained that:\qt{this represents children's conception of stories at their age, which is why I believe it holds greater significance to present it in a realistic manner}.

\textbf{Family Meaning Co-constructing.} We noticed that family meaning co-constructing is another preferred quality for parents to support in HCI. First, the storybooks co-created by families can be used as family memory archiving, e.g, \qt{I believe the storybook from P2' developmental phase contribute to mirror her mindset, and I think it is really meaningful~(P17)}. T1 also expressed that as the accumulated stories can \qt{witness the growth of children}, and these stories can \qt{reflect what the children care about at the moment} and \qt{be considered valuable assets for family memory archiving}. Moreover, parents demonstrated that storymaking as a family bonding becomes family activities. For example, P9 described that crafting stories becomes one of their family activities using AI-printed materials:\qt{during the Dragon Boat Festival, she and her father made a story book together, and his father was responsible for writing. She said it was a gift, and she will make an interesting storybook for her birthday}. Storymaking as a family bonding activity can strengthen relationships, foster creativity, and create a sense of togetherness~\cite{wajskop2015dramatic}.

\subsubsection{Therapists' Needs}
In this section, we reported three themes for therapists' needs:(1) Observing and Understanding the Strength and Challenges of Children and Family; (2) Moderating Family Communication through Storymaking; (3) Offering a Playful and Safe Space.

\textbf{Observing and Understanding the Strength and Challenges of Children and Family.} 
In our findings, we found that therapists need to observe and understand the strength and challenges of children and family. Specifically, the following three aspects need to be supported:(1) understanding children's strengths; (2) discovering the challenges of family communication.

First, therapists need to understand children's strengths during the activities. T1 understood the strengths of each family’s children through stories and story characters, e.g, \qt{through the character of Xixi, I think P2 is a very kind child. When Shoushou said he had no friends to play with, she thought she would play with him.[...] He was injured, so she took him to see a doctor. She is actually a kind-hearted child who cares about others}. Additionally, T1 can better understand the child's strengths through P10's interaction with AI:\qt{AI did not present the images she wanted, and she would flexibly adjust her thoughts to accept this imperfection. So, that flexibility was particularly good, and she was very calm and friendly during the whole process}. When T1 observe the child's characteristics, the therapist might further strengthen these strengths:\qt{for example, when we discovered children's strengths during this activities, I might repeat them to the child}. According to positive psychotherapy theory\cite{rashid2015positive}, this strength-based approach can help therapist identify and capitalize on children's strengths to face challenges.

Furthermore, therapists can discover the challenges of family communication. Therapists can understand the challenges of family communication through storytelling and story characters:\qt{In P2's story, she said that she didn't want to take medicine, which actually means that she understood the truth, but she didn't like it from her heart~(T1)}. T1 can understand the interactions of family through making during the process of parents and children interacting with AI:\qt{when the children and parents chose the four images generated by AI. I observed that parents and children discussed together to choose which images they liked and which images they didn't like. I could understand their interactions in this process}. T2 added that: \qt{a child made a lot of small gifts for his mother, such as small cakes and biscuits. The mother disliked them very much, so the therapist could also understand how they interact at home. The therapist's primary role is to facilitate our observation of natural family interactions. Art activities serve as a medium. Through making arts, we might understand how parents and children communicate with each other, and how they deal with conflicts of opinions}.

\textbf{Moderating Family Communication through Storymaking.} One of interesting theme from therapists is to moderate family communication through storymaking. It involved three aspects: (1) facilitating communication through role-playing; (2) facilitating communication through perspective-taking; (3) facilitating communication through co-creation.

First, therapists can encourage children to use their story characters to foster role-playing to communicate with each others. During the activity, after the AI generated their own characters, T1 encouraged the children to \qt{name characters} and used the story characters they created to express their thoughts and experiences:\qt{P1 created a little bunny, and I helped her put herself into this character. I went to visit her castle with her through the story}. Children can express their thoughts and concerns more comfortably through role-playing, leading to open and honest conversations\cite{carpenter1982using}. 

Second, therapists can facilitate children and parents to communicate with each other through perspective-taking. T1 tended to encourage family members switch roles using AI-printed materials or character tokens during the activities:\qt{I encouraged the child to play the role of his angry mother. What does the mother say and why does the mother think that way?}.  P3 became aware of how the child perceived their communication through switching their roles:\qt{from my perspective, I believe I engaged in reasoned communication with him, avoiding gabbling something. However, from his perspective, he perceived my communication as gabbling something. I think the content of the communication is very important, but the content of the communication is not so important to him}. Facilitating perspective-taking can help families overcome egocentric tendencies, promote mutual understanding, and consequently cultivate harmonious relationships\cite{ohtaka2019perspective}.

Third, therapists can facilitate communication through co-creation. T2 stated the demands of traditional family expressive arts therapy activities:\qt{parents don't know how to participate in co-creation with their children. Another challenge is that parents tend to tell their children what to do. Thus, I think how to balance the participation of parents and children in this process}. In our activities, T1 encouraged parents and children to co-create through turn-taking:\qt{T1 suggested that I could create one, and P4 also crafted one. The idea was to later integrate our creations using AI, which I found quite impressive. This represented a pattern of initially individual creation followed by co-creation~(P3)}.

\textbf{Offering a Playful and Safe Space.} 
In our study, we found that it is important to creating a playful and safe space for therapists. First, therapists need to support a playful and relaxing space for children and parents. T3 explained that the family story-making was \qt{a process of play}, and play \qt{allows us to better release our personality so that we can be ourselves}. T1 observed the importance of a playful and relaxing environment to a child's state: \qt{I remember one time P16 was humming a song while cutting and collaging by himself. This emotional state deeply moved me}. Therapists can help parents return to a state of innocence through providing diverse materials. For example, P5 noted that she felt relaxed using clay:\qt{In terms of clay, I bought it for my children many times. I never played it myself, but I played with clay this time}. Meanwhile, parents' relaxed state also affects the state of the child:\qt{The more you relax and enjoy the process, the more relaxed your child will be~(T1)}. Furthermore, P3 interpreted a safe space as \qt{a loving environment}, which can children express themselves freely, because \qt{everyone accepted to him and allowed him to dare to express themselves freely without concerns}. The safe space might create an environment where participants feel comfortable while engaging in the creative process and expressing their thoughts\cite{lazar2018making}.

\begin{table*}[tb]
\caption{Summary of the Needs from Children, Parents and Therapists.}
\centering
\vspace{-3mm}
\label{tab:finding1need}
\small
\begin{tabular}{m{1cm} m{4cm} m{5cm} m{7.5cm}}
\hline
Roles& Needs &Description &Example Quotes \\
\hline
\multirow{5}{*}{Children}
&
Diverse Material for Creative Exploration and Expression
& \begin{itemize}
\item Self-regulation and motor skills; 
\item Non-verbal expression;
\item Creative empowerment.
\end{itemize}  
& 
\begin{itemize}
\item \qt{While kneading clay, my son was really focused~(P5)}; 
\item \qt{Half of the children could tell stories in their drawings~(T4)}.
\item \qt{So, he rarely built such a thing creatively by himself~(P17)}.
\end{itemize} 
\\
&
Authentic Encounter with Reality
& 
\begin{itemize}
\item The incorporation of real characters into stories; 
\item The incorporation of personal objects into stories.
\end{itemize}   
& 
\begin{itemize}
\item \qt{He said that the seahorse is the mother and the jellyfish is the father~(P11)}; 
\item \qt{When these toys were integrated into his stories, he might perceive them as more than mere playthings, and thus the toy might connect with the child~(P17)}.
\end{itemize}
\\
&
Parental Involvement
& 
\begin{itemize}
\item Parents serve as a role model; 
\item Common topics co-construction.
\end{itemize}
& 
\begin{itemize}
\item \qt{I guess he felt mommy focused on making her own thing, and thus I should focus on making my own thing too~(P3)};
\item \qt{Ocean themes are also of interest to his dad}.
\end{itemize}
\\
&
Sense of Accomplishment
&
\begin{itemize}
\item Children's joy at creating results that exceeded expectations; 
\item Sharing their storybook.
\end{itemize}
&
\begin{itemize}
\item \qt{She felt that she actually couldn't draw such a good-looking character~(P1)};
\item \qt{He told his friends I was going to AI today~(P11)}.
\end{itemize}
\\
&
Renarration Beyond Activities
&
\begin{itemize}
\item Continuing making new stories in home.
\end{itemize}
&
\begin{itemize}
\item \qt{She used those AI pictures to make this storybook again~(P1)};
\end{itemize}
\\
\hline
\multirow{4}{*}{Parents}
&
Discovering New Aspects of Children
& \begin{itemize}
\item  Discovering children's demands for parents; 
\item  Discovering children's less noticeable life experiences;
\item  Discovering children's strenghts.
\end{itemize}  
& 
\begin{itemize}
\item \qt{So when the purple fish~(created by the child) felt cold, he went to the seahorse because the seahorse gave him a sense of security~(P11)}; 
\item \qt{I realized that she might feel that kindergarten life for her is happy and enjoyable~(P9)}.
\item \qt{Parents need to amplify their children's strengths consistently, transforming them into shining points~(T1)}.
\end{itemize} 
\\
&
Learn from the Therapist
& \begin{itemize}
\item  Learning how to accept and minimize judgment towards their children; 
\item  Learning how to nurture children's imagination.
\end{itemize}  
& 
\begin{itemize}
\item \qt{I think it was great when the therapist guided her to imagine~(F9)}; 
\end{itemize} 
\\
&
Reflection in Therapeutic Storymaking
& \begin{itemize}
\item  Reflecting on their roles; 
\item  Reflecting their family interactions;
\item  Reflecting on their own results-oriented expectations.
\end{itemize}  
& 
\begin{itemize}
\item \qt{At home, I paid more attention to my children's affairs, often taking on a controlling or guiding role~(P3)}; 
\item \qt{It seems that families engage in few collaborative play activities together~(P5)}; 
\item \qt{In the process of co-creation together, I always felt that P2's story plot was too simple~(P1)}.
\end{itemize} 
\\
&
Family Meaning Co-constructing
& \begin{itemize}
\item  Family memory archiving; 
\item  Storymaking as a family bonding.
\end{itemize}  
& 
\begin{itemize}
\item \qt{It can witness the growth of children~(T1)}; 
\item \qt{During the Dragon Boat Festival, she and her father made a story book together~(P9)}.
\end{itemize} 
\\
\hline
\multirow{3}{*}{Therapists}
&
Observing and Understanding the Strength and Challenges of Children and Family
& \begin{itemize}
\item  Understanding children's strengths; 
\item  Discovering the challenges of family communication.
\end{itemize}  
& 
\begin{itemize}
\item \qt{Through the character of Xixi, I think P2 is a very kind child~(T1)}; 
\item \qt{Through making arts, we might understand how parents and children communicate with each other, and how they deal with conflicts of opinions~(T2)}.
\end{itemize} 
\\
&
Moderating Family Communication through Storymaking
& \begin{itemize}
\item  Facilitating communication through role-playing; 
\item  Facilitating communication through perspective-taking;
\item  Facilitating communication through co-creation.
\end{itemize}  
& 
\begin{itemize}
\item \qt{P1 created a little bunny, and I helped her put herself into this character~(T1)}; 
\item \qt{I encouraged the child to play the role of his angry mother~(T1)}; 
\item \qt{T1 suggested that I could create one, and P4 also crafted one. The idea was to later integrate our creations using AI~(P3)}.
\end{itemize} 
\\
&
Offering a Playful and Safe Space
& \begin{itemize}
\item  Supporting a playful and relaxing space; 
\item  Supporting a safe space.
\end{itemize}  
& 
\begin{itemize}
\item \qt{Play allows us to better release our personality so that we can be ourselves~(T3)}; 
\item \qt{Everyone accepted to him and allowed him to dare to express themselves freely without concerns~(P3)}.
\end{itemize} 
\\
\hline

\end{tabular}
\end{table*}










==> texfiles/6-Findings2.tex <==
\section{Findings 2}
In the second part of the study, we aimed at how AI could be used as an art material in family expressive arts therapy. Our qualitative research analysis reveals how AI-infused materials and physical materials support family expressive art therapy at different levels of the ETC framework and the therapeutic meanings that AI materials hold within the context of family expressive therapy.
\subsection{Understanding Material Interactions with AI as a Lens of ETC}
In this section, we examine how text-to-image tools as art materials can support family art therapy activities. Material and media interactions play a pivotal role in the the therapeutic outcomes and the overall experience of the clients\cite{lazar2018making}. Within this domain, the Expressive Therapies Continuum(ETC) is an important framework which classifies how clients interact with art materials to process information and form images from simple to complex\cite{hinz2019expressive}.
It provides four dimensions, including Kinesthetic/Sensory level, Perceptual/Affective level, Cognitive/Symbolic level, and Creative level.
We employed ETC as a lens to examine various media interactions within our activities from these four dimensions. These media interactions included the mutual transformation and integration of AI materials and physical materials(see \autoref{fig:etc}).
\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{images/etc.jpeg}
  \vspace{-4mm}
  \caption{.}
  \Description{}
  \label{fig:etc}
\end{figure*}
\subsubsection{Kinesthetic/Sensory Level.} At the Kinesthetic/Sensory Level, the processing of information commences at a preverbal stage\cite{hinz2019expressive}. The Kinesthetic component encompasses the sensations that provide individuals with information about bodily rhythms, movements, and actions\cite{hinz2019expressive}. The Sensory component~(S) encompasses information derived from visual, auditory, and tactile channels\cite{hinz2019expressive}. On the Kinesthetic component~(K), we found that children used to engage in physical manipulation and handling of various materials through movement and actions, such as pounding clay with their hands (P4, see \autoref{fig:etc}~\circled{1}), cutting out AI printed characters (P13, see \autoref{fig:etc}~\circled{2})), moving rhythmically with acrylic stands made by AI (P18), pushing (P2,P4,P16), stabbing and cutting clay (P4), and cutting non-woven fabric (P2, P10, P13). According to theories, these activities can facilitate individuals’ release of energy, physical arousal, and tension\cite{kagin1978expressive}. It also promotes relaxation for clients\cite{slater2004healing}. As noted by P5, \qt{The clay is still very cool, and it seems to be quite relaxing}.
On the Sensory component, we found that parents and children explored the sensory qualities of various materials through tactile, visual, and auditory exploration. For example, P4 used a board with wooden texture (see \autoref{fig:etc}~\circled{3}), and also P17 used what she described as a soft, translucent toy during the session (see \autoref{fig:etc}~\circled{4}). According to theories, these activities can enhance broader attention to the present moment, encourage self-soothing, and express inner sensation.

\subsubsection{Perceptual/Affective Level}
At the Perceptual/Affective Level, information processing and image formation transpire, sometimes without reliance on words\cite{hinz2019expressive}. 
The Perceptual component~(P) deals with images and expressions through a focus on the formal elements(line, size or color) of visual representation\cite{hinz2019expressive}. 
At the Affective end of this level~(A), information processing can manifest as emotional and raw, translating into images characterized by vibrant colors\cite{hinz2019expressive}.
On the Perceptual component, we found that family members tended to create images through form, boundaries and containment, and pattern using structural materials~(e.g, wood, LEGO®, colored pencils, and AI-printed materials). 
For instance, P16 organized the LEGO® with a high degree of form potential in a visual order~(see \autoref{fig:etc}~\circled{7}). Children used different sizes of AI-printed characters to collage on the board~(P4, P10 and P16), and P10 formed a row of AI-printed characters in the classroom scene~(see \autoref{fig:etc}~\circled{8}). According to theories, these activities might increase structural awareness and foster a satisfying internal state\cite{ulman2001art,hinz2019expressive}. 
On the side of the Affective component, we found that children used vibrant and dark colors using clay and AI-printed materials~(P4, P8, P16 and P18). P8 employed a combination of different vibrant colors, rule-breaking shapes and form distortions to evoke his emotion~(see \autoref{fig:etc}~\circled{5}). Large size snake with bright green color was utilized by P7 to express her anger~(see \autoref{fig:etc}~\circled{6}). These activities might help children access emotions through providing fluid mediums and encouraging the use of intense and deep colors\cite{hinz2019expressive}.

\subsubsection{Cognitive/Symbolic level}
At the Cognitive/Symbolic level, processing information is complex and sophisticated, involving planning, cognitive action, and intuitive recognition\cite{hinz2019expressive}. 
At the Cognitive of this level~(C), it is thought processes including planning, logical thought, problem-solving, reality-directed information processing, and storytelling\cite{hinz2019expressive}.
At the Symbolic of this level~(Sy), it involves intuitive, mythical and self-oriented creation of concepts, and the articulate expression and resolution of symbolic elements\cite{hinz2019expressive}.
On the Cognitive component, we found that children could plan and sequence their story plots with their parents through narratives and collages~(P2,P7,P10,P13,P16,and P18). F16 employed AI-printed collages to distribute food to different characters logically through selection, organization and calculation~(see \autoref{fig:etc}~\circled{10}). P10 employs problem-solving skills to address various injuries that arise within her storybook~(see \autoref{fig:etc}~\circled{9}). Thus, it might increase planning, cause and effect thinking, and problem-solving skills~\cite{hinz2019expressive}.
On the Symbolic component, we found that all children choose their favorite toys and made story characters to connect stories and concrete individual experiences through metaphoric symbols. For instance, a little rabbit character was constructed as a self-symbol through AI and was integrated into P2's own story. At the same time, this story character was integrated into the child's life in the form of a physical symbolic material~(see \autoref{fig:etc}~\circled{22}). The family members of F5 respectively made their own characters as a self-symbol, and the tortoise toy as a metaphorical symbol of security were integrated into the story through AI~(see \autoref{fig:etc}~\circled{11}). Thus, it might help children realize personal meaning and help parents expand their knowledge about child through personal symbols\cite{kagin1978expressive,hinz2019expressive}.

\subsubsection{Creative level}
At the Creative level~(Cr), it involves innovative and resourceful interactions with the environment, including art materials, that lead to creative and self-actualizing experiences\cite{hinz2019expressive}. 
It can ``bring forth something new'' within the expressive process across all levels of ETC. 
For example, at the Kinesthetic/Sensory Level, P4 employed a variety of colored pens to create rhythmic trajectories on the paper though body movements without purpose, and at the same time uses sensations to understand the trajectories similar to tornadoes~(see \autoref{fig:etc}~\circled{13}). 
At the Perceptual/Affective level,  ; 
At the Cognitive/Symbolic level, P4 created a magical plane metaphorically in the process of developing the story to help parents creatively solve the problem of lost diamonds(see \autoref{fig:etc}~\circled{15}). Thus, these activities might lead to creative self-actualizing experiences\cite{hinz2019expressive}.

\subsection{Understanding the Therapeutic Meaning of AI as Art Material}
In this section, we aim to understand the therapeutic meaning of AI as art materials in family expressive art therapy. Our findings revealed three themes~(see Table~\ref{tab:finding2ai}): (1) AI as Empowerment for Family; (2) AI as the Connection Between Physical and Digital, Life and Story; (3) AI as a Family Collaborator. 

\subsubsection{AI as Empowerment for Family}
The notion of employing AI as a art material holds two forms of empowerment dynamic within family-based expressive art therapy: (1) AI can lower the art-making threshold threshold and increase creation efficiency; (2) AI can empower children's imagination.

\textbf{AI can Lower the Art-making Threshold and Increase Creation Efficiency.} In our findings, we found that AI can lower the art-making threshold threshold through enhancing the aesthetic quality of creation. For example, P1 elucidates the appeal of AI-generated outcomes that exceed expectations, especially for children:\qt{P2 said that the tool is so magical, which makes the rabbit so beautiful. What left the most indelible impression on her was that Xixi became beautiful, the castle was so beautiful, and the car was so beautiful}. Thus, creating sophisticated and high-quality images can help children and parents boost expressive confidence and focus on approaching creation rather than outcomes :\qt{children could become bolder in their creative pursuits, knowing that the quality of their drawing doesn't matter as much since AI can improve and enhance it. It made it more realistic and adding backgrounds to enrich the atmosphere~(P17)}. Furthermore, AI can help parents and children increase their creation efficiency. For example, P3 examined that:\qt{If I were to attempt to create an oil painting with this effect, it would demand an investment of three days to a week and considerable effort. Yet, exceptional results can be rapidly attained through the utilization of two wooden blocks}. Through increasing their creation efficiency, it might boost creativity for improvisation and foster creative freedom\cite{barclay1999magic}.

\textbf{AI can Empower Children's Imagination.} 
Many parents demonstrated that AI can unconditionally embrace the imaginative world of children. For example, P11 noted that:\qt{he might envision such a scene in his mind but may struggle to articulate it due to his current language proficiency. Nevertheless, these images support him to imagine. I observed him wearing a continuous smile as he watched the images. While he may not have verbally expressed it, he radiated happiness inwardly. This was the scene he wanted}. T3 explained that AI is meaningful for promoting children’s imagination through integrating physical art materials:\qt{ children is given the opportunity to mold an animal from clay or draw a bridge, and then generate them using AI. I think it can enhance the child's imagination}. Thus, embracing children's imagination can help to foster creative self-expression, and psychological self-healing and renewal\cite{mcniff1992art}.

Second, AI provides rich options and endless possibilities for children and parents. It can offer families with multiple options by generating different variations:\qt{AI offers many choices while also making selections within specific categories~(P3)}. In addition,P17 mentioned that AI might create more possibilities when using certain materials:\qt{manipulating colored clay or working with Lego can be even more unpredictable, yielding unexpected surprises. What you end up with might not exactly match your initial vision, that's perfectly acceptable. In contrast, AI can generate even more unforeseen possibilities}. Therefore, rich options and endless possibilities for children and parents might drive parents and children more exploration in the therapeutic settings~\cite{brandle2023empowerment}. Also, it can promote communication between parents and children:\qt{children and parents made choices based on 4 AI-generated images. Some children clearly expressed their likes and dislikes, and also some parents and children discussed and chose together. This phenomenon sheds light on the interaction between parents and children during this selection process~(T1)}.

\begin{table*}[tb]
\caption{Summary of the Therapeutic Meaning of AI as Art Materials.}
\centering
\vspace{-3mm}
\label{tab:finding2ai}
\small
\begin{tabular}{m{4cm} m{5cm} m{6.5cm}}
\toprule 
Themes &Description &Example Quotes \\
\midrule
AI as Empowerment for Family
& \begin{itemize}
\item AI can lower the art-making threshold threshold and increase creation efficiency; 
\item AI can empower children's imagination.
\end{itemize}  
& 
\begin{itemize}
\item \qt{Children could become bolder in their creative pursuits, knowing that the quality of their drawing doesn't matter as much since AI can improve and enhance it}; 
\item \qt{These images support him to imagine}.
\end{itemize} 
\\
AI as the Connection Between Physical and Digital, Life and Story
& 
\begin{itemize}
\item AI facilitates the mix of different materials; 
\item AI material promotes play and performance;
\item AI creates symbols that can permeate life and stories.
\end{itemize}   
& 
\begin{itemize}
\item \qt{We made a building block, made a colored clay, and drew a few pictures, and then AI generated such a beautiful image}; 
\item \qt{AI create some character tokens, and you could role play};
\item \qt{She has immersed herself in this role}.
\end{itemize}
\\
AI as a Family Collaborator 
& 
\begin{itemize}
\item Human-AI dialogue between verbal and non-verbal expression; 
\item AI inspires children's creative interpretation;
\item Dynamic human-AI comprise and authorship.
\end{itemize}
& 
\begin{itemize}
\item \qt{The child provided a concept or crafted an original object, and then AI could process it};
\item \qt{I may be able to recreate based on the AI-generated images};
\item \qt{AI provided several images and allowed them to choose one that closely mirrored their own creation. This may be considered as respecting their ideas}.
\end{itemize}
\\
 \bottomrule
\end{tabular}
\end{table*}

\subsubsection{AI as the connection between physical and digital, life and story.} 
In this study, we found that AI as a art material can foster the connection between physical world and digital world, and real life and story. It involved three categories: (1) AI facilitates the mix of different materials; (2) AI material promotes play and performance; (3) AI creates symbols that can permeate life and stories.

\textbf{AI Facilitates the Mix of Different Materials.} We found that AI facilitates the mix of different materials. 
AI can integrate art elements created by parents and children using different physical materials, which promotes collaboration between parents and children. 
For example, P1 described that:\qt{we made a building block, made a colored clay, and drew a few pictures, and then AI generated such a beautiful image}. 
Also, therapists believed that AI as an art material can \qt{shuttles} between the physical and the digital world, e.g, \qt{I noticed that children initially made colored clay, which were tactile, three-dimensional. Additionally, they could draw or build their own scenes. The AI-generated images were not necessarily final outcomes, and they could be brought to 3D physical world to recreate~(T4)}. Thus, it could foster the continuity of their human creations:\qt{children can witness that their artworks have different dimensions. AI can make these artworks reused and then recreated repeatedly. I personally think it is very attractive to children}.

\textbf{AI Material Promotes Play and Performance.} In our study, many parents mentioned that AI material promotes play and performance during family expressive art therapy. AI-printed materials could help children tell stories though moving these materials flexibly during expressive art therapy:\qt{after cutting these AI-printed materials, he used them when he wanted to tell stories. Children might be clear about where objects should be placed and how these characters should be played. As an example, when these characters slept, P13 flipped them over. I think this is very important~(P11)}. T3 think AI material help children better take on the role:\qt{AI create some character tokens, and you could role play. Children might immerse themselves in embodying those roles}. The embodiment of AI enhances the flexibility and playfulness of expressive art therapy, thereby increasing the creativity of improvisation.

\textbf{AI Creates Symbols that can Permeate Life and Stories.} In our study, AI could help children creates symbols that can permeate life and stories. First, AI could help children constructed self-symbols based on their creation, and integrate self-symbols into children's own stories. For example, P1 noted that:\qt{she has immersed herself in this role because she felt that the little rabbit itself was something we created at the time. Now, she identifies her current state with the character of Xixi(the little rabbit)}. Constructing self-symbols can help children reflect their qualities represented in them\cite{hinz2019expressive}.

Furthermore, physical materials(e.g, AI-printed materials and physical character tokens ) created by AI were brought into real life, serving as transitional objects. Transitional object is typically defined as an item to which a child forms a notably strong attachment during childhood~\cite{winnicott1951transitional}. In expressive art therapy, T4 explained that the definition of transitional object:\qt{when clients leave the therapy studio, they can take a piece of their creation with them, which can help them reflect back on their experience in expressive art therapy. It bridges the gap between the therapeutic environment and the real world, facilitating the extension of therapeutic gains and personal growth into everyday life}. For our children participants, P17 described that the physical character tokens were taken home to play with other toys in the physical world:\qt{he used those tokens as his toys and other toys to play with}. Thus, AI materials as transitional objects might provide a sense of comfort, security, and emotional support to a child~\cite{winnicott1951transitional}.

\subsubsection{AI as a Family Collaborator.} An interesting theme from AI is that AI as a family collaborator has three therapeutic aspects: (1) human-AI dialogue between verbal and non-verbal expression; (2) AI inspires children's creative interpretation; (3) dynamic human-AI comprise and authorship. 

\textbf{Human-AI Dialogue between Verbal and Non-verbal Expression.} AI enables the bridging of verbal and non-verbal expression, akin to the core essence of expressive art therapy:\qt{the underlying logic of expressive arts therapy is the transformation of images into languages. Initially, you need to create art,  which involves the operation of your right brain. Then, the left hemisphere engages when you share your creations through storytelling. This transition facilitates the journey of inner thoughts and emotions from from your subconscious a process of consciousness}. In terms of AI, it accepts linguistic and visual inputs, promoting a holistic mode of expression, and mitigating the challenges associated with verbal communication. Our video analysis data showed that many children described this creation under the guidance of the therapist after completing their own creation: \qt{what do you think this is? A house? A castle? Or a character?~(T1)}. Then, AI could generate images based on their descriptions and creations. Also, many parents mentioned that AI can assist children in converting abstract concepts into concrete representations, e.g, \qt{The child provided a concept or crafted an original object, and then AI could process it. For example, he made a pile of mud and put it there, and AI could even create specific characters, which was quite impressive~(P3)}.

\textbf{AI Inspires Children's Creative Interpretation.} In our study, children gave new interpretations based on AI-generated content. T4 explained that these fresh interpretations are indeed processes of meaning-making: \qt{what's interesting to me is that not only did he choose the AI-generated variation of the banana image, but he also named the banana that called it the jeweled banana. He actively engaged in the process of meaning-making. If I were there, I would think that moment is very important}. The children's creative interpretation of AI were incorporated into the subsequent phase of their making process:\qt{AI has generated some materials. I can actually make stories directly from the perspective of the materials. I may be able to recreate based on the AI-generated images, which was quite interesting.[...] For example, I didn't make trees when I was creating, because I noticed the trees generated by AI, and then I could use the trees to stimulate new thinking and creativity~(P3)}.

\textbf{Dynamic Human-AI Comprise and Authorship.} Interestingly, in our study, when the images generated by AI were not similar to artworks created by children, most children tended to choose to compromise with the results generated by AI. For example, P17 explained that:\qt{initially, we probably had a preconceived notion, but when AI generated images that deviated from our expectations, we found this variation to be acceptable. Moreover, we engaged in interpreting the  the meaning behind the AI-generated images, aiming to identify similar images}. Human-AI comprise might mean that children can embrace the imperfections of AI artworks:\qt{when it comes to children, one point we may need to pay attention to is why the children think the artwork is not perfect, and then how the children can accept this imperfection and still coexist with the artwork. I think this is a relatively subtle part~(T2)}. Children-AI comprise might foster a sense of acceptance and self-compassion~\cite{dreikurs1959courage}.

Further, human-AI authorship is essential in expressive arts therapy. T4 used the relationship between the creator and the creation in expressive art therapy to explain the importance:\qt{I find myself intrigued by the dynamics of authorship between the creator and the AI-generated images. In expressive art therapy, an individual creates a drawing, and regardless of its aesthetic appeal, they often say, 'this is my artwork.' However, when AI generates an image that they find beautiful, will they similarly claim authorship and confidently proclaim, 'this is my creation,' when sharing it with others?}. In our study, many parents mentioned that children thought they made the story themselves:\qt{she created this story herself, and she also came up with this character~(P1)}. P5 explained that providing more choices can help establish human-AI authorship:\qt{AI provided several images and allowed them to choose one that closely mirrored their own creation. This may be considered as respecting their ideas}.














